Bias Field Poses a Threat to DNN-based X-Ray Recognition

The chest X-ray plays a key role in screening and diagnosis of many lung diseases including the COVID-19. More recently, many works construct deep neural networks (DNNs) for chest X-ray images to realize automated and efficient diagnosis of lung diseases. However, bias field caused by the improper medical image acquisition process widely exists in the chest X-ray images while the robustness of DNNs to the bias field is rarely explored, which definitely poses a threat to the X-ray-based automated diagnosis system. In this paper, we study this problem based on the recent adversarial attack and propose a brand new attack, i.e., the adversarial bias field attack where the bias field instead of the additive noise works as the adversarial perturbations for fooling the DNNs. This novel attack posts a key problem: how to locally tune the bias field to realize high attack success rate while maintaining its spatial smoothness to guarantee high realisticity. These two goals contradict each other and thus has made the attack significantly challenging. To overcome this challenge, we propose the adversarial-smooth bias field attack that can locally tune the bias field with joint smooth & adversarial constraints. As a result, the adversarial X-ray images can not only fool the DNNs effectively but also retain very high level of realisticity. We validate our method on real chest X-ray datasets with powerful DNNs, e.g., ResNet50, DenseNet121, and MobileNet, and show different properties to the state-of-the-art attacks in both image realisticity and attack transferability. Our method reveals the potential threat to the DNN-based X-ray automated diagnosis and can definitely benefit the development of bias-field-robust automated diagnosis system.

==> related_backup.tex <==
\section{Related Work}\label{sec:related}
% In this section, we will summarize the related works including X-Ray imagery recognition, noise-based adversarial attack and the adversarial attack on medical imagery.
% \felix{TODO}

%-------------------------------------------------------------------------
\subsection{X-Ray Imagery Recognition}
%
% emphasize on Chest X-Ray imagery only. 
% emphasize on recognition accuracy
%
% although DNNs are powerful, the robustness to medical imaging degradation, \eg, bias field, are rarely explored. This paper is very first work from the view of adversarial attack.

% \felix{common noise degradation are rarely found in X-ray imagery. In practice, the kind of degradation pertains to the X-ray imagery is commonly known as the bias field, which is xxx xxx xxx. In this work, we capitalize on this proprietary degradation surrounding X-ray imagery and initiate adversarial attacks based on imperceptible modification on the bias field itself.} 

X-ray radiography is widely used in the medical field for diagnosis or treatment of diseases. In recent years, many public X-ray image datasets are made available, leading to a wide literature examining data mining or deep learning techniques on such datasets.

One of the largest datasets is the ChestX-ray14 dataset from the National Institutes of Health (NIH) Clinical Center, which contains over 108,948 frontal-view X-ray images with 14 thoracic diseases, and  other non-image features. Together with the dataset, \cite{Wang2017CXRDataset} evaluates the performance of 4 classic convolutional neural network (CNN), namely AlexNet, ResNet-50, VGGNet, and GoogLeNet, on the multi-label image classification of diseases, creating an initial baseline of average area under the ROC curve (AUC) of 0.745 over all 14 diseases.

Inspired by this work, many researchers starts utilising the power of deep neural network on chest X-ray (CXR) classification. \cite{Li2017} presents a framework to jointly perform disease classification and localisation. With the use of bounding box to predict lesion area location, the classification performance is improved to an average AUC of 0.755. \cite{yao2017} proposes the use of a CNN backbone with a variant of DenseNet model, combining with a long-short term memory network (LSTM) to exploit statistical dependencies between labels, achieving an average AUC of 0.761. \cite{GUAN2020259} explores a category-wise residual attention learning (CRAL) framework, which is made up of feature embedding and attention learning module. Different attention weights are given to enhance or restrain different feature spatial regions, yielding an average AUC score of 0.816. \cite{Rajpurkar2017} proposes the use of transfer learning by fine-tuning a modified DenseNet , resulting in an algorithm called CheXNet, a 121 layer CNN. It further raises the average AUC  to 0.842. \cite{Guan2018} presents the use of a three- branch attention guided CNN, which focuses on local cues from (small) localized lesion areas. The combination of local cues and global features achieves an average AUC achieves 0.871. 
The state of the art results using the official spilt released by \cite{Wang2017CXRDataset} are held by \cite{Gundel2018} with average AUC of 0.817. The paper argues that when random spilt is used, the same patient is likely to appear in both train and test set, and this overlap affects performance comparison. The method proposed is a location aware DenseNet-121, trained on ChestXRay14 data and PLCO dataset, which incorporates the use of spatial information in high resolution images.

The power of deep learning techniques on CXR is also explored for detection of COVID-19, motivated by the need of quick, effective and convenient screening.  Studies showed that some COVID-19 patients displayed abnormalities in their CXR images. \cite{COVIDwang2020} releases an open access benchmark dataset COVIDx along with COVID-Net, a deep CNN designed for detection of COVID-19 from CXR images, achieving a sensitivity of 97.3 and appositive predict value of 99.7. Many studies have also leverage on variant of the dataset and network for prediction of COVID-19 \cite{COVIDafshar,COVIDli,COVIDTertaglione}.

Despite the strong performance of DNN, and considerations made to address data irregularities like class imbalance in dataset, the effect of medical image degradation on disease identification was rarely investigated and addressed. For example, bias field, also referred to as intensity inhomogeneity, is a low frequency smooth intensity signal across images due to imperfections in image acquisition methods. Bias field could adversely affect quantitative image analysis \cite{Juntu2005BiasField} Many inhomogeneity correction strategy are hence proposed in the literature \cite{brey1988correction}\cite{fan2003unified}\cite{thomas20053d}.

However, the possible detrimental effect on disease identification, location or segmentation by the bias field are rarely explored in literature, hence DNN proposed may not be robust towards this inherent degradation. To the best of authors' knowledge, this paper is very first work that looks at the effect of bias field from the view of adversarial attack.


%-------------------------------------------------------------------------
\subsection{General Adversarial Attack}

Despite the robustness of various DNN deployed in solving different recognition problems in image, speech or natural language processing application, many studies have shown that DNN are susceptible to adversarial attacks \cite{szegedy2013intriguing}\cite{goodfellow2014explaining}. There exist many literatures that propose different adversarial attacks, and they can be generally classified into attacks in training and testing stage.

In training stage, attackers can carry out data poisoning, which involves the insertion of adversarial example into training dataset, affecting model’s performance. For example, poison frog leverages on inserting images into dataset to ensure the wrong classification will be given to a target test sample \cite{shafahi2018poison}. The use of direct gradient method in generating adversarial images against neural network is also explored \cite{yang2017generative}.

In testing stage, attackers can carry out either white-box or black-box attacks. In white-box attacks, attackers are assumed to have access to target classifier. \cite{biggio2013evasion} focuses on optimising discriminant function to mislead a 3 layer full connected neural network. \cite{shafahi2018poison} suggests that a certain imperceptible perturbation can be applied to cause misclassification on image, and this effect can be transferred to other different network to train on similar data to misclassify the same input. Fast gradient sign method (FGSM) is proposed by \cite{goodfellow2014explaining}. It involves only one back propagation step when calculating the gradient of cost function, hence allowing fast adversarial example generation \cite{kurakin2016adversarial} proposes the iterative version of FGSM, known as basic iteration method (BIM), which heuristically search for examples that are most likely to fool the classifier. Given the presence of literature that defends against FGSM methods, \cite{carlini2017towards} proposes the use of margin loss instead of entropy loss during attacks. \cite{cisse2017houdini} proposes a an approach named HOUDINI, which generate adversarial examples for fooling visual and speech recognition models. Instead of altering pixel values, spatial transformed attacks are also proposed to perform special transformation such as translation or rotation on images \cite{xiao2018spatially}.

In black box attacks, attackers have no access to classifier's parameter or training sets. \cite{papernot2017practical} proposes the exploitation of transferability of adversarial examples. A model similar to the target classifier is first trained, then adversarial examples generated to attack the trained model is used to target the actual classifier. \cite{fredrikson2015model} explores the exploitation of knowledge of confidence value of target classifier as predictions are made. 

% \qing{1. noise pattern not exist, 2. few medical degradation-based attack 3. bias field widely exist. no one do this}

%-------------------------------------------------------------------------
\subsection{Adversarial Attack (and Defense) on Medical Imagery}
There are existing literature that looks into adversarial attack against deep learning system for medical imagery. \cite{finlayson2018adversarial} shows that both black box and white box PGD attack and adversarial patch attack could affect the performance of classifiers modelled after state-of-the-art systems on fundoscopy, chest X-ray and dermoscopy respectively. Similarly, \cite{paschali2018generalizability} also shows that small perturbation can create classification performance drop across state-of-the-art networks such as Inception and UNet, for which accuracy drops from above 87\% on normal medical images to almost 0\% on adversarial examples. By producing crafted mask, an adaptive segmentation mask attack (ASMA) is proposed to fool DNN model for segmenting medical imagery \cite{ozbulak2019impact}.

In medical adversarial defence, \cite{li2020defending} proposes an unsupervised detection of adversarial samples in which unsupervised adversarial detection (UAD) are complemented with semi-supervised adversarial training (SSAT). The proposed model claims to demonstrate a superior performance in medical defence against other techniques. \cite{ma2020understanding} further proposes that medical DNN are more vulnerable to attacks due to the specific characteristic of medical images having high gradient regions sensitive to perturbations, and over parameterization of the state-of-the-art DNN. This work then proposes an adversarial detector specifically designed for medical image attacks, achieving over 98\% detection AUC. 

However, very few literature has leverage on and conduct adversarial attack based on the inherent characteristic of the targeted medical imagery. For example, common noise degradation used for general adversarial attacks are rarely found in X-ray imagery. Hence in this work, we capitalize on the proprietary degradation surrounding X-ray imagery, bias field, and initiate adversarial attacks based on imperceptible modification on the bias field itself.

